Modeling Hierarchical Spaces: A Review and Unified Framework for Surrogate-Based Architecture Design

Simulation-based problems involving mixed-variable inputs frequently feature domains that are hierarchical, conditional, heterogeneous, or tree-structured. These characteristics pose challenges for data representation, modeling, and optimization. This paper reviews extensive literature on these structured input spaces and proposes a unified framework that generalizes existing approaches. In this framework, input variables may be continuous, integer, or categorical. A variable is described as meta if its value governs the presence of other decreed variables, enabling the modeling of conditional and hierarchical structures. We further introduce the concept of partially-decreed variables, whose activation depends on contextual conditions. To capture these inter-variable hierarchical relationships, we introduce design space graphs, combining principles from feature modeling and graph theory. This allows the definition of general hierarchical domains suitable for describing complex system architectures. Our framework defines hierarchical distances and kernels to enable surrogate modeling and optimization on hierarchical domains. We demonstrate its effectiveness on complex system design problems, including a neural network and a green-aircraft case study. Our methods are available in the open-source Surrogate Modeling Toolbox (SMT 2.0).

==> FM.tex <==
\usetikzlibrary{angles,shadows.blur,positioning,backgrounds,arrows.meta}
\forestset{
  declare count register=disjuncts from,
  disjuncts from'=0,
  declare count register=concrete from,
  concrete from'=2,
  concrete colour/.code={\colorlet{concretecol}{#1}},
  abstract colour/.code={\colorlet{abstractcol}{#1}},
  draw colour/.code={\colorlet{drawcol}{#1}},
  concrete colour=gray,
  abstract colour=white,
  draw colour=black,
  /tikz/mandatory/.style={circle, fill=drawcol, draw=drawcol},
  /tikz/optional/.style={circle, draw=drawcol, fill=white},
  /tikz/concrete/.style={fill=concretecol, draw=drawcol},
  /tikz/abstract/.style={fill=abstractcol, draw=drawcol},
  /tikz/or/.style={},
  mandatory/.style={edge label={node [mandatory] {}}},
  optional/.style={edge label={node [optional] {}}},
  or/.style={for first={disjunct}},
  disjunct/.style={
    tikz+={\path (.parent) coordinate (A) -- (!u.children) coordinate (B) -- (!ul.parent) coordinate (C) pic[draw, angle radius=2.5ex] {angle};}
  },
  disjunction tree/.style={
    where={isodd(n_children())}{
      for n={int((n_children()+1)/2)}{calign with current},
    }{
      calign=midpoint,
    },
    before typesetting nodes={
      for nodewalk={
        filter/.wrap pgfmath arg={{level>=##1}{n_children()>1}}{(disjuncts_from)}
      }{
        or,
      },
      where={level()>=(concrete_from)}{
        concrete,
      }{
        abstract,
      },
%
    },
    for tree={
      parent anchor=children,
      child anchor=parent,
      l'+=10mm,
      blur shadow,
      rounded corners,
      text height=2ex,
      text depth=.5ex,
      font=\sffamily,
    },
  },
}
\bgroup
\sbox0{%
\begin{forest}% addaswyd o gôd Salim Bou: https://tex.stackexchange.com/a/335782/
  disjunction tree,
  disjuncts from'=1,
  concrete from'=1,
  concrete colour=blue!85!cyan!40,
  abstract colour=blue!85!cyan!15,
  draw colour=darkgray,
  [Multi-Layer Perceptron 
    [Learning rate, mandatory]
    [Optimizer,  mandatory
      [ASGD
      [Decay]
      [Power upd.]
      [Avg. start]
      ]
      [Adam
      [Run. avg. 1]
      [Run. avg. 2]
      [Num. stab.]
      ]
    ]
    [Hidden layers, optional
      [Lay. $1$ units \# ]
      [$\ldots$]
      [Lay. $l$ units \#]
    ]
     [Dropout, optional
        [Small val.]
      [High val.]
      [Any val.]
    ]
    [Activation function, mandatory
      [ReLU]
      [Sigmoid]
      [Tanh]
    ]
  ]
%\draw[dashed,latex-latex] (-7,-2) -- (-1.4,-2);
%
\draw[dashed,-latex] (-11.1,-4.1) -- (-1.4,-2);
\draw[dashed,-latex] (-3.65,-4.1) -- (-1.4,-2);
%
%\draw[dashed,-latex] (1.4,-2) -- (14.2em,-2);
%
\draw[dashed,-latex] (0.4,-4.1) -- (14.2em,-2);
\draw[dashed,-latex] (-0.6,-4.1) -- (14.2em,-2);
\draw[dashed,-latex] (3.4,-4.1) -- (14.2em,-2);
%
\draw   (-1ex,-2.5) coordinate (A) -- (0,-2.4) coordinate (B) -- (1ex,-2.5) coordinate (C) pic[fill=drawcol, angle radius=2.5ex] {angle};
\end{forest}}%


%
\sbox1{\begin{tabular}{clclcl}
\tikz{\draw (0,0) node[circle,fill=black,inner sep=.5ex] (A) {} (A.north) -- (0,2ex);} & Mandatory &
\tikz{\draw (0,0) coordinate(A) -- (2ex,2ex) coordinate(B) -- (4ex,0) coordinate(C)
  pic[draw, angle radius=1.5ex] {angle=A--B--C};} & Alternative &
\tikz{\draw[dashed,-latex] (0,0) (0,1ex) -- (2em,1ex);} & Requires \\
\tikz{\draw (0,0) node[circle,draw,inner sep=.5ex] (A) {} (A.north) -- (0,2ex);} & Optional &
\tikz{\draw (0,0) coordinate(A) -- (2ex,2ex) coordinate(B) -- (4ex,0) coordinate(C)
  pic[fill=black, angle radius=1.5ex] {angle=A--B--C};} & Or &
\tikz{\draw[dashed,latex-latex] (0,0) (0,1ex) -- (2em,1ex);} & Excludes \\
\end{tabular}}%
%
\begin{tikzpicture}
  \node (forest){\usebox0};
  \node[below=2ex,draw,rounded corners] at (forest.south) {\usebox1};
\end{tikzpicture}
\egroup


==> func.tex <==
\vspace{3pt}
\begin{forest}
      for tree={
        font= \small \ttfamily,
        grow'=0,
        child anchor=west,
        parent anchor=south,
        anchor=west,
        calign=first,
        inner xsep=10pt,
        inner ysep = -3pt,
        edge path={
          \noexpand\path [draw, \forestoption{edge}]
          (!u.south west) +(7.5pt,0) |- (.child anchor)  \forestoption{edge label};
        },
        % style for your file node 
        file/.style={edge path={\noexpand\path [draw, \forestoption{edge}]
          (!u.south west) +(7.5pt,0) |- (.child anchor) \forestoption{edge label};},
          inner xsep=2pt, inner ysep=-3pt ,font=\footnotesize \ttfamily
                     },
        before typesetting nodes={
          if n=1
            {insert before={[,phantom]}}
            {}
        },
        fit=band,
        before computing xy={l=15pt},
      }  
    [ \   \normalsize \texttt{SMT 2.0}
     % [config
     % ]
      [ \textcolor{blue}{Sampling methods}
        [Random, file
        ]      
        [Full Factorial, file
        ]
        [ Latin Hypercube Sampling \textcolor{Orchid}{(Nested LHS and Extended LHS)}, file
        ]
      ]
      [ \textcolor{blue}{Problems}
        [Aircraft wing weight, file
        ]      
        [Robot arm position, file
        ]  
        [Water flow through a borehole, file
        ]   
        [Low frequency torsion vibration, file
        ]    
        [Welded beam shear stress, file
        ]  
        [ \textcolor{Orchid}{Mixed integer cantilever beam}, file
        ]
        [ \textcolor{Orchid}{Hierarchical neural network}, file
        ]      
      ]
      [ \textcolor{blue}{Surrogate modeling methods}
        [ RBF: Radial Basis Functions, file
        ]
        [IDW: Inverse-Distance Weighting, file
        ]
        [RMTS: Regularized Minimal-energy Tensor-product Splines, file
        ]
         [LS: Least-Squares approximation, file
        ]      
         [QP: Quadratic Polynomial approximation,  file
        ]
        [Kriging based models,  file
            [Continuous kernels,  file]
            [\textcolor{Orchid}{Hierarchical kernels},  file]
            [\textcolor{Orchid}{Categorical kernels},  file]
            %    [Kriging: Gaussian Process interpolation,  file]
             %   [KPLS: Kriging with Partial Least Squares,  file]
            %    [KPLSK: Kriging with Partial Least Squares+Kriging,  file]
           %     [GEKPLS: Gradient-Enhanced Kriging with Partial Least Squares,  file]
        ]
        [\textcolor{Orchid}{GENN: Gradient-Enhanced Neural Network},  file ]
         [ \textcolor{Orchid}{MGP: Marginal Gaussian Process},  file ]
      ]
      [ \textcolor{blue}{Applications}
          [   Mixture of experts (MOE) , file]
          [  Variable-fidelity modeling (VFM) , file]
          [  Multi-fidelity Kriging (MFK) , file]
         [    \textcolor{Orchid}{ Multi-fidelity KPLS (MFKPLS)} , file]
         [    \textcolor{Orchid}{ Multi-fidelity KPLSK (MFKPLSK)} , file]
         [   Efficient Global Optimization (EGO) , file]
         [  \textcolor{Orchid}{ Mixed-Integer and hierarchical usage surrogates}, file]
      ]
        [ \textcolor{blue}{Interactive notebooks}
          [  SMT tutorial for surrogate modeling, file]
          [  \textcolor{Orchid}{  Noisy Gaussian process (Kriging) }, file]
          [ \textcolor{Orchid}{Multi-fidelity Gaussian process (with or without noise)} , file]
         [  \textcolor{Orchid}{ Gaussian process trajectory Sampling} , file]
         [ \textcolor{Orchid}{ Bayesian optimization to solve unconstrained problems} , file]
         [ \textcolor{Orchid}{ Mixed \& hierarchical Kriging and optimization}, file]
      ]
    ]
 \end{forest}
